Leveraging Outdoor Webcams for Local Descriptor Learning

We present AMOS Patches, a large set of image cut-outs, intended primarily for the robustification of trainable local feature descriptors to illumination and appearance changes. Images contributing to AMOS Patches originate from the AMOS dataset of recordings from a large set of outdoor webcams. The semiautomatic method used to generate AMOS Patches is described. It includes camera selection, viewpoint clustering and patch selection. For training, we provide both the registered full source images as well as the patches. A new descriptor, trained on the AMOS Patches and 6Brown datasets, is introduced. It achieves state-of-the-art in matching under illumination changes on standard benchmarks.

==> Figs/fig_patches.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[max width=0.5\textwidth]{Imgs/patches.png}
    \caption{Examples of AMOS patches. Each column contains a subset of patches from a patch set.}
    \label{fig:patches}
\end{figure}
% The results are averaged over 3 runs.
